Deviation results for sparse tables in hashing with linear probing

We consider the model of hashing with linear probing and we establish the moderate and large deviations for the total displacement in sparse tables. In this context, Weibull-like-tailed random variables appear. Deviations for sums of such heavy-tailed random variables are studied in \cite{Nagaev69-1,Nagaev69-2}. Here we adapt the proofs therein to deal with conditioned sums of such variables and solve the open question in \cite{TFC12}. By the way, we establish the deviations of the total displacement in full tables, which can be derived from the deviations of empirical processes of i.i.d.\ random variables established in \cite{Wu94}..

==> commath.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commandes mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{babel}					%Pour les commandes dépendant de la langue du document
\RequirePackage{amsmath}				%Math de l'AMS
\RequirePackage{amssymb}				%Autres symboles mathématiques
\RequirePackage{amsthm}					%Théorèmes correctement organisés
\RequirePackage{bbm}					%Fonction indicatrice
\RequirePackage{stmaryrd}				%Crochets pour les intervalles entiers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Rémi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Making \big, etc. a relative size rather than absolute (with default parameters, ex is 4.3045 pt)
%
%\renewcommand\big[1]{{\hbox{$\left#1\vbox to 1.97ex{}\right.\n@space$}}}
%\renewcommand\Big[1]{{\hbox{$\left#1\vbox to 2.67ex{}\right.\n@space$}}}
%\renewcommand\bigg[1]{{\hbox{$\left#1\vbox to 3.37ex{}\right.\n@space$}}}
%\renewcommand\Bigg[1]{{\hbox{$\left#1\vbox to 4.07ex{}\right.\n@space$}}}
%
%% Paired delimiters
%
%\DeclarePairedDelimiter\abs\lvert\rvert % Absolute value
%\DeclarePairedDelimiter\brack\lbrack\rbrack % Brackets
%\DeclarePairedDelimiter\ceil\lceil\rceil % Ceiling
%\DeclarePairedDelimiter\floor\lfloor\rfloor % Floor
%\DeclarePairedDelimiter\intervalicc\llbracket\rrbracket % Closed integer interval
%\DeclarePairedDelimiter\intervalico\llbracket\llbracket % Closed-open integer interval
%\DeclarePairedDelimiter\intervalioc\rrbracket\rrbracket % Open-closed integer interval
%\DeclarePairedDelimiter\intervalioo\rrbracket\llbracket % Open interger interval
%\DeclarePairedDelimiter\norm\lVert\rVert % Norm
%\DeclarePairedDelimiter\paren() % Parentheses
%\DeclarePairedDelimiter\set\{\} % Set
%
%\DeclarePairedDelimiterX\inner[2]\langle\rangle{#1,#2} % Inner product
%\DeclarePairedDelimiterX\intervalcc[2]\lbrack\rbrack{#1,#2} % Closed interval
%\DeclarePairedDelimiterX\intervalco[2]\lbrack\rparen{#1,#2} % Closed-open interval
%\DeclarePairedDelimiterX\intervaloc[2]\lparen\rbrack{#1,#2} % Open-closed interval
%\DeclarePairedDelimiterX\intervaloo[2]\lparen\rparen{#1,#2} % Open interval
%\DeclarePairedDelimiterX\setst[2]\{\}{#1\ \delimsize|\ #2} % Set of the #1 such that #2
%
%% Use of some characters from the Fourier-GUTenberg package
%
%\DeclareFontEncoding{FMS}{}{}
%\DeclareFontSubstitution{FMS}{futm}{m}{n}
%\DeclareFontEncoding{FMX}{}{}
%\DeclareFontSubstitution{FMX}{futm}{m}{n}
%\DeclareSymbolFont{fouriersymbols}{FMS}{futm}{m}{n}
%\DeclareSymbolFont{fourierlargesymbols}{FMX}{futm}{m}{n}
%\DeclareMathDelimiter{\llbracket}{\mathopen}{fouriersymbols}{153}{fourierlargesymbols}{133}
%\DeclareMathDelimiter{\rrbracket}{\mathclose}{fouriersymbols}{154}{fourierlargesymbols}{134}
%\DeclareMathDelimiter{\VERT}{\mathord}{fouriersymbols}{152}{fourierlargesymbols}{147}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mathématiques générales
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ensembles de nombres
\newcommand{\ensnombre}[1]{\mathbb{#1}}%
\newcommand{\N}{\ensnombre{N}}
\newcommand{\Z}{\ensnombre{Z}}
\newcommand{\Q}{\ensnombre{Q}}
\newcommand{\R}{\ensnombre{R}}
\newcommand{\C}{\ensnombre{C}}

%Divers
\newcommand{\card}[1]{\left\lvert #1 \right\rvert}

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\dom}{dom}


\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norme}[1]{\left\lVert #1 \right\rVert}
\newcommand{\prodscal}[2]{\left\langle {#1} \mathrel{}\middle|\mathrel{} {#2} \right\rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\ensfonction}[3]{#1(#2 ; #3)}
\newcommand{\enstq}[2]{\left\{ #1 \mathrel{}\middle|\mathrel{} #2 \right\}}
\newcommand{\ensavec}[2]{\left\{ #1\ ;\ #2 \right\}}
\newcommand{\enspart}{\mathfrak{P}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{\mathrel{=}:}

\newcommand{\seq}[1]{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Algèbre linéaire
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ensmatrice}[3]{\mathcal{#1}_{#2}(#3)}

\newcommand{\transposee}[1]{{#1}^\top}
%\newcommand{\transposee}[1]{{}^t\! #1}

\DeclareMathOperator{\rg}{rg}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Com}{Com}
\DeclareMathOperator{\Mat}{Mat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Probabilités
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\indic}{\mathbbm{1}}
\DeclareMathOperator{\Leb}{Leb}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Loi}{\mathcal{L}}
\newcommand{\Espe}{\mathbb{E}}
\newcommand{\ET}{\sigma}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\newcommand{\complementaire}[1]{#1^\mathsf{c}}

\newcommand{\Probcond}[2]{\Prob\left( #1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Loicond}[2]{\Loi\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Especond}[2]{\Espe\left[ #1 \mathrel{}\middle|\mathrel{} #2 \right]}
\newcommand{\Varcond}[2]{\Var\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}




\iflanguage{french}%
{
%VERSION FRANCAISE

\DeclareMathOperator{\Vect}{Vect}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\cosh\relax
\DeclareMathOperator{\cosh}{ch}
\let\sinh\relax
\DeclareMathOperator{\sinh}{sh}
\let\tanh\relax
\DeclareMathOperator{\tanh}{th}

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\arcosh}{argch}
\DeclareMathOperator{\arsinh}{argsh}
\DeclareMathOperator{\artanh}{argth}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator*{\supess}{sup\,ess}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2\mathclose{}\mathpunct{},#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{]}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{[}}%
\newcommand{\intervalleoo}[2]{\intervalle{]}{#1}{#2}{[}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Théorème}%
\newtheorem{lemma}{Lemme}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollaire}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Propriété}%
\newtheorem{properties}{Propriétés}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Définition}%
\newtheorem{hypothesis}{Hypothèse}%
\newtheorem{example}{Exemple}%
\newtheorem{examples}{Exemples}%
\newtheorem*{exercise}{Exercice}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remarque}%
\newtheorem*{plus}{Complément}%
\newtheorem*{question}{Question}%
\theoremstyle{plain}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Topologie
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\interieur}{int}
\DeclareMathOperator{\adherence}{adh}
}
{
%VERSION ANGLAISE

\DeclareMathOperator{\Vect}{span}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\artanh}{artanh}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator*{\supess}{ess\,sup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2,#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{(}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{)}}%
\newcommand{\intervalleoo}[2]{\intervalle{(}{#1}{#2}{)}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%\newcounter{intervallent}%
%\newcommand{\intervallentff}[2]{%
%	\setcounter{intervallent}{#1}%
%	\stepcounter{intervallent}%
%	\left\{#1,\theintervallent,\dots,#2\right\}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}%
\newtheorem{lemma}{Lemma}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollary}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Property}%
\newtheorem{properties}{Properties}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Definition}%
\newtheorem{hypothesis}{Hypothesis}%
\newtheorem{example}{Example}%
\newtheorem{examples}{Examples}%
\newtheorem*{exercise}{Exercise}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remark}%
\newtheorem*{plus}{Plus}%
\newtheorem*{question}{Question}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Topologie
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\interieur}{int}
\DeclareMathOperator{\adherence}{cl}
}
